GS-Marker: Generalizable and Robust Watermarking for 3D Gaussian Splatting

In the Generative AI era, safeguarding 3D models has become increasingly urgent. While invisible watermarking is well-established for 2D images with encoder-decoder frameworks, generalizable and robust solutions for 3D remain elusive. The main difficulty arises from the renderer between the 3D encoder and 2D decoder, which disrupts direct gradient flow and complicates training. Existing 3D methods typically rely on per-scene iterative optimization, resulting in time inefficiency and limited generalization. In this work, we propose a single-pass watermarking approach for 3D Gaussian Splatting (3DGS), a well-known yet underexplored representation for watermarking. We identify two major challenges: (1) ensuring effective training generalized across diverse 3D models, and (2) reliably extracting watermarks from free-view renderings, even under distortions. Our framework, named GS-Marker, incorporates a 3D encoder to embed messages, distortion layers to enhance resilience against various distortions, and a 2D decoder to extract watermarks from renderings. A key innovation is the Adaptive Marker Control mechanism that adaptively perturbs the initially optimized 3DGS, escaping local minima and improving both training stability and convergence. Extensive experiments show that GS-Marker outperforms per-scene training approaches in terms of decoding accuracy and model fidelity, while also significantly reducing computation time.

==> bak/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> bak/_1_intro.tex <==
\section{Introduction}
\label{sec:intro}
\ca{teaser: input GS->NN->distort->decode. generalizable (multi object), distorted.}
\begin{figure}
  \centering
   \includegraphics[width=0.99\linewidth]{Figs/teaser.pdf}
   \caption{The Proposed WaterGS Pipeline.}
  \label{fig:teaser}
\end{figure}
3D technologies play a crucial role in various fields, such as the film and gaming industries, augmented reality (AR), virtual reality (VR), and medical imaging \cite{}. Resent advancements in 3D Gaussian splatting \cite{} have significantly expanded the frontiers of 3D representation. This technique utilizes a set of 3D Gaussian primitives to model objects or scene in 3D space, and incorporates the differentiable rendering algorithm to render images under certain camera poses. The two characteristics of 3D Gaussian splatting, explicit representation and differentiable rendering, allow it to emerge as a sophisticated method of 3D representation, offering real-time rendering capabilities and unparalleled flexibility in editing. Despite the widespread study and application of 3D Gaussian splatting, there remains a notable gap in the research concerning issues of copyright protection for 3D Gaussian splatting.

% Digital watermarking is a widely adopted technique for protecting the ownership and security of digital asserts. In this domain, numerous existing works have introduced robust watermarking approach for 2D image, such as HiDDeN \cite{} and MBRS \cite{}. To ensure the security of 3D Gaussian splatting, an intuitive solution may be to apply these existed 2D image watermarking techniques to the rendered images of 3D Gaussian splatting. However, while this approach embeds watermark messages in the rendered images, it fails to secure the ownership of the 3D Gaussian splatting model itself. If the 3D Gaussian splatting is illicitly obtained, new images can be generated without the embedded watermark, resulting in a breach of ownership claims. Therefore, a more effective approach to protect the ownership of 3D Gaussian splatting models would involve embedding the watermark directly into the 3D Gaussian splatting itself, allowing for the extraction of the embedded watermark message from the subsequently rendered 2D images. This method would ensure that the ownership is preserved across both the model and its rendered images.

Digital watermarking is a widely adopted technique for protecting the ownership and security of digital asserts. In this domain, numerous existing works have introduced robust watermarking approach for 3D models. These watermarking methods varying significantly depending on the 3D representation. For mesh and point cloud models, which represent 3D objects explicitly through vertices and points, the mainstream approach usually involves directly embedding and extracting watermark message on the vertex and points. In contrast, for Neural Radiance Fields (NeRF), which represent 3D scenes or models implicitly through a neural field, a typical watermarking method involves intergrating the watermark message into the neural field and extracting the embedded message from the rendered images of the watermarked NeRF. Although these method are robust and effective, they are not compatible with 3D Gaussian splatting. On the one hand, most applications of 3D Gaussian splatting involve the use of rendered images, thus the watermark messages are expected to be extracted from these rendered images rather than the 3D Gaussian splatting itself. Therefore, the watermarking methods designed for 3D mesh and point cloud models are unsuitable for 3D Gaussian splatting. On the other hand, 3D Gaussian splatting represents scene and objects explicitly with 3D Gaussian primitives, contrasting with NeRF's implicit representation. In addition, most watermarking algorithms designed for NeRF require significant computational resources and training time to fine-tune the NeRF model with the watermark message, making them less flexible for practical applications. Therefore, the watermarking methods designed for NeRF are also unsuitable for 3D Gaussian splatting. 

% To address this problem, we aim to design a watermarking algorithm for 3D Gaussian splatting. An intuitive solution to achieve that may be to apply these existed 2D image watermarking techniques to the rendered images of 3D Gaussian splatting. However, while this approach embeds watermark messages in the rendered images, it fails to secure the ownership of the 3D Gaussian splatting model itself. If the 3D Gaussian splatting is illicitly obtained, new images can be generated without the embedded watermark, resulting in a breach of ownership claims. Therefore, a more effective approach to protect the ownership of 3D Gaussian splatting models would involve embedding the watermark directly into the 3D Gaussian splatting itself, allowing for the extraction of the embedded watermark message from the subsequently rendered 2D images. This method would ensure that the ownership is preserved across both the model and its rendered images.



To address the aforementioned problem, we propose a novel watermarking framework, WaterGS, specifically designed specially for 3D Gaussian splatting. As illustrated in Fig.~\ref{fig.teaser}, the proposed framework utilizes a 3D PointNet-based encoder to embed the watermark message into the input 3D Gaussian splatting, followed by a 2D CNN-based decoder that extracts the watermark message from the rendered images of the watermarked Gaussian splatting. To facilitate the embedding of watermark messages, we design a strategy that incorporates random Gaussian primitives into the input Gaussian splatting. This strategy enables the model to achieve a better balance between bit accuracy and visual quality. Our WaterGS is characterized by three key features. First, the embedding process of our WaterGS is \textbf{generalizable} for any given 3D Gaussian splatting. Our model can embed the watermark message into the input Gaussian splatting through a unify pipeline, eliminating the need for per-input optimization and thus enabling a generalizable and efficient embedding process. Secondly, WaterGS is \textbf{robust} against various forms of distortion, with the decoder capable of accurately extracting the watermark message even when the rendered images have been subjected to corruption or degradation. Finally, the watermark messages embedded by our WaterGS are \textbf{invisible}, ensuring that the watermarked Gaussian splatting is virtually indistinguishable from the input Gaussian splatting.

Our contributions are summarized as follows:
\begin{itemize}
    \item We design a generalizable and robust framework, WaterGS, for watermarking 3D Gaussian splatting. To the best of our knowledge, we are the first to design a generalizable watermark framework specifically for 3D Gaussian splatting. Our WaterGS can watermark any given 3D Gaussian splatting without per-input optimization, thereby circumventing the substantial computational resources typically required for fine-tuning 3D models.
    \item We design a strategy to introduce random Gaussian primitives into the input Gaussian splatting during the embedding process, thereby achieving an optimal balance between bit accuracy and visual quality.
    \item We conduct extensive experiments to validate the effective of our proposed WaterGS framework.
\end{itemize}


==> bak/_3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/_1_intro_cvpr.tex <==
% \cb{
\section{Introduction}
\label{sec:intro}
\begin{figure}
  \centering
   \includegraphics[width=0.99\linewidth]{Figs/teaser_v2.pdf}
   % \caption{The Proposed WaterGS Pipeline. \ca{images are too small, remove distortion layer, 3d encoder can be small}}
   \caption{(a). The 2D encoder-decoder-based watermarking framework. (b). The proposed WaterGS framework. Inspired by the 2D watermarking framework, we design a novel encoder-decoder framework for watermarking 3DGS. The proposed WaterGS framework is generalizable across any given 3D model and messages. The residual ($\times 10$) of rendered images between the input and watermarked 3DGS demonstrates that WaterGS embeds watermark with minimal impact on the visual quality of 3DGS.}
  \label{fig:teaser}
\vspace{-10pt}
\end{figure}

% In the generative AI landscape, there has been a rapid proliferation of digital assets generated by AI, including images, videos, 3D models, and model weights. Besides, advancements in 3D reconstruction techniques, such as Neural Radiance Fields (NeRF) \cite{nerf} and 3D Gaussian Splating (3DGS) \cite{3dgs}, have significantly boosted the growth of 3D models. In this context, safeguarding the copyright protection of digital assets has become increasingly vital.
Within the generative AI landscape, the swift increase in AI-generated digital assets has made the protection of copyright for the digital assets more critical than ever. 
Invisible watermarking, which embeds watermarks without compromising the original assets' quality, has emerged as an effective and popular solution. 2D methods (\cref{fig:teaser} (a)), such as \cite{hidden}, have shown great success by utilizing an encoder-decoder framework to embed and extract messages in images. 2D methods have proven to be efficient and generalizable across a wide array of images and embedded messages. 


However, extending 2D methods to accommodate 3D models presents substantial challenges, indicating a clear gap in the existing technology. Securing 3D models requires protecting their 2D renderings. This requires the watermarks to be embedded within 3D models, but extractable from the 2D projections. Intuitively, the encoding process must be compatible with specific 3D representations, such as meshes, Neural Radiance Fields (NeRF) \cite{nerf}, and 3D Gaussian splatting (3DGS) \cite{3dgs}. There are a few methods have been developed for mesh and NeRF. Mesh-based techniques \cite{mesh_watermark1,mesh_watermark2,mesh_watermark3} employ complex algorithms to insert watermarks into the vertices and textures, resulting in sophisticated encoding processes. NeRF-based methods \cite{copyrnerf,waterf,nerf_watermark1} incorporate watermarks within the radiance field by a time-consuming fine-tuning procedure of the original NeRF model. 
3DGS has recently emerged as a leading representation for rendering. However, only a single recent study, GS-Hinder \cite{gs_hider}, has explored steganography within 3DGS, which hides messages within 3DGS via per-scene optimization. Yet, this method is impractical for watermarking a large volume of 3D models due to its significant time requirements. As 3DGS becomes a dominant form, there is an urgent need for a watermarking approach that can efficiently handle any model and any message without extensive per-scene training.

In this paper, we propose a novel framework, \textbf{WaterGS}, for the generalizable and robust watermarking for 3DGS, capable of embedding watermarks in a single forward pass, illustrated in \cref{fig:teaser} (b). To ensure the generalizability and robustness, we face two challenges: 1) developing a 3DGS encoder that can effectively generalize across diverse models, and 2) ensuring the accuracy of watermark extraction from free-view renderings subjected to various distortions.

WaterGS consists of a 3D encoder for message embedding within 3DGS and a 2D decoder for message extraction from renderings. These components are jointly optimized to enhance the decoding accuracy while maintaining high rendering fidelity. For the embedding process, the encoder employs a residual prediction strategy, which makes minor adjustments to the original assets, diverging from conventional 2D methods \cite{hidden}. However, naively perturbing the geometry or texture could potentially impair the model integrity, given that the original 3DGS is typically optimized. Inspired from the splitting operation utilized in classic 3DGS optimization \cite{3dgs}, a technique that facilitates escaping local minima in optimization, we introduce an innovative yet simple approach. We propose a minimal set of additional Gaussian primitives dedicated to watermarking tasks. These primitives, which we term as W-Markers, are strategically spread throughout the model to ensure comprehensive coverage. Following this, the W-Markers along with the input model are processed via an embedding network. This network utilizes a point-based architecture, aimed at enabling the efficient and effective embedding of watermarks. The strategic placement of W-Markers not only simplifies the concurrent goals of message embedding and model fidelity preservation but also crucially enables the extraction of messages from any projected view of the 3D model. Furthermore, WaterGS is enhanced to be robust against various distortions, with the decoder capable of accurately extracting the messages even when the rendered images have corruption or degradation. 
% Finally, WaterGS framework demonstrates remarkable efficiency, capable of embedding a watermark message with a single forward pass. We evaluate the watermarking embedding time between our framework and other 3D watermarking methods. Our method successfully embeds a watermark message into 3DGS in less than one second using an NVIDIA GeForce RTX 3090 GPU. In contrast, the existing watermarking method for NeRF, known as WateRF \cite{waterf}, necessitates more than 60 minutes to complete the same task. This difference in time efficiency is primarily attributed to the extensive fine-tuning process required by WateRF.



In summary, our contribution is three-fold.
\begin{itemize}
\item 
We present WaterGS, the first framework to offer a generalizable and robust solution for the invisible watermarking of 3DGS. Distinguished by its ability to watermark any 3DGS without the need for per-input training, WaterGS highly reduces the extensive computational cost. 
% We evaluate the watermarking embedding time for our framework in comparison to other 3D watermarking methods. Our method embeds the watermark message into 3DGS model within one second using a NVIDIA GeForce RTX 3090 GPU. In contrast, the existed watermarking method for NeRF, WateRF, requires more then 60 minutes to complete the embedding due to the extensive fine-tuning process. 
%  We evaluate the watermarking embedding time for our framework compared with other 3D watermarking methods. Our method embeds watermark message into 3DGS within 1s in a NVIDIA GeForce RTX 3090 GPU, while the existed watermarking method for NeRF, WateRF, requires more then 60mins due to the fine-tuning process. 
\item 
We introduce the W-Markers proposal, a novel approach that advancing the embedding process, making it both affordable and efficient. This method facilitates in striking an optimal balance between decoding accuracy and model fidelity.
\item
% We demonstrate the performance of WaterGS through comprehensive experiments. Our results show that it achieves superior accuracy and model fidelity compared to the more time-intensive methods that require per-scene training.
We demonstrate the performance of WaterGS through comprehensive experiments. Our results show that it achieves superior accuracy and model fidelity compared to existing methods that require per-scene training.
\end{itemize}

\todos{rewrite, shorten intro}

% }




==> sec/_3_method_cvpr.tex <==
\section{Method}
\label{sec.method}


\paragraph{Overview.}
We propose a novel framework for embedding watermark messages into 3D objects parameterized by 3DGS. Our approach enables watermark embedding into 3DGS models and extracts the embedded message from the corresponding rendered images. 
% The proposed framework is $(i)$ \emph{generalizable}, capable of embedding watermark message into any given 3D object parameterized by 3DGS in a single forward pass; $(ii)$ \emph{invisible}, ensuring the watermarked 3D Gaussian splatting remains visually similar to the original; $(ii)$ \emph{robust}, with the decoder exhibiting resilience to noise and disturbances. 
As demonstrated in \cref{fig:pipeline}, our framework is composed of three key modules: a) an encoder that embeds the watermark message into 3DGS; b) a distortion layer that enhances the robustness of the proposed framework; c) a decoder that retrieves the embedded message from the rendered images. \todos{rewrite}

In the subsequent section, we will first provide a brief introduction on the symbol definitions used in our method in \cref{sec.method_definitions}. We will then introduce the 3D encoder in \cref{sec.method_3D_encoder}, the distortion layer in \cref{sec.method_distortion_layer}, and the 2D decoder in \cref{sec.method_2D_decoder}. We will finally detail the training process in \cref{sec.method_loss_funs}.
 % We will detail these components in the subsequent section. 

\subsection{Definitions}
\label{sec.method_definitions}
Our framework is specifically designed for watermarking 3DGS. In formal terms, 3DGS represents a 3D model as a set of Gaussian primitives. Each Gaussian primitive $\mathcal{G}$ is characterized by its center position $\mu \in\mathbb{R}^3$, scaling factor $s\in\mathbb{R}^3$, and rotation quaternion $q \in \mathbb{R}^4$. In 3D space, the fundamental function of a Gaussian primitive is defined as:
\begin{equation}
    \mathcal{G} = \text{e}^{-\frac{1}{2}(x - \mu)^T\Sigma^{-1}(x-\mu)}
    \label{Gaussian}
\end{equation}
where the covariance matrix $\Sigma$ is derived from the scaling factor $s$ and rotation quaternion $q$. During the rendering process, the color of Gaussian primitives is determined by the opacity $\alpha \in \mathbb{R}$ and spherical harmonic (SH) coefficients $h\in\mathbb{R}^{3\times (k+1)^2}$, where $k$ represents the order of SHs. 

In our watermark framework, we define the input 3DGS that consists of $N$ Gaussian primitives as $G_{in}(M_{in}, S_{in}, Q_{in}, C_{in}, A_{in})$, where $M_{in}\in\mathbb{R}^{N\times 3}$, $S_{in}\in\mathbb{R}^{N\times 3}$, $Q_{in}\in\mathbb{R}^{N\times 4}$, $C_{in}\in\mathbb{R}^{N\times (3\times (k+1)^2)}$, $A_{in}\in\mathbb{R}^{N}$ represent the center position, scaling factor, rotation quaternion, color, and opacity of the $N$ Gaussian primitives, respectively. The binary message of length $l_b$ to be embedded into the Gaussian splatting is denoted as $M \in \{0, 1\}^{l_b}$.

\input{sec/w_marker}

\subsection{Network Design}
\paragraph{3D Encoder}
\label{sec.method_3D_encoder}
Given the input Gaussian splatting $G_{in}$ consisted of $N$ Gaussian primitives, we employ a 3D encoder for watermark embedding. The working pipeline of the proposed 3D encoder is demonstrated in \cref{fig:pipeline}. Specifically, we first design a specially random Gaussian splatting, termed \textbf{W-Markers}, and integrate it into the input Gaussian splatting. The incorporation of the W-Markers introduces random textures into the input Gaussian splatting, thereby enhancing the efficacy of watermark message embedding. Subsequently, an \textbf{embedding network} is employed to receive the textured Gaussian splatting and the message $M$ as input, and generates the watermarked Gaussian splatting $G_{wm}$. In this section, we provide a detailed explanation of the design and implementation of the embedding pipeline. 
% Given the input Gaussian splatting $G_{in}$ that consisted of $N$ Gaussian primitives, we employ a 3D encoder for watermark embedding. The working pipeline of the proposed 3D encoder is demonstrated in \cref{fig:pipeline}. Specifically, w e first design a W-Markers initialization process to pre-process the input Gaussian splatting. This process incorporates random texture into the input Gaussian splatting, thereby enhancing the efficacy of watermark message embedding. 
% % This pre-process will add  \textit{W-Marker} into the input Gaussian primitives. The W-Markers consisted of $N_{W}$ random Gaussian primitives, which can facilitate watermark message embedding.
% % introduce $N_r$ random Gaussian primitives into the input Gaussian splatting. The random Gaussian primitives, named as \textit{W-Marker}, can introduce random texture into the 3D models, which is able to facilitate watermark message embedding. 
% Subsequently, an embedding network is employed to integrate the watermark message into the input Gaussian splatting. The embedding network receives the textured Gaussian splatting and the message $M$, as input, and outputs the watermarked Gaussian splatting $G_{wm}$. In this section, we provide a detailed explanation of the design and implementation of the embedding pipeline. 
% Then, we concatenate the center position, scaling, rotation, opacity and color attribution of the 3DGS to construct a Gaussian tensor $G_t \in \mathbb{R}^{(N+N_r) \times (11 + 3\times (k+1)^2)}$. Next, we replicate each bit of the message $N$ times to form a message tensor $M_t \in \mathbb{R}^{(N+N_r)\times N_b}$. The message tensor is then concatenated with the Gaussian tensor $G_t$, resulting in a combined tensor $G_m \in \mathbb{R}^{(N+N_r)\times (11 + 3\times (k+1)^2 + N_b)}$. We employ a PointNet architecture \cite{} for the encoder, which takes the combined tensor $G_m$ as input and output the watermarked Gaussian splatting $G_{wm}$. 

% the 3D encoder takes as input the 3DGS $G_{in}$ and the message $M$, producing as output the watermarked 3D Gaussians splatting $G_{wm}$. In the encoding process, we first concatenate the center position, scaling, rotation, opacity and color attribution of the 3DGS to construct a Gaussian tensor $G_t \in \mathbb{R}^{N \times (11 + 3\times (k+1)^2)}$. Next, we replicate each bit of the message $M$ $N$ times to form a message tensor $M_t \in \mathbb{R}^{N\times N_b}$. The message tensor is then concatenated with the Gaussian tensor $G_t$, resulting in a combined tensor $G_m \in \mathbb{R}^{N\times (11 + 3\times (k+1)^2 + N_b)}$, which serves as the input to our proposed encoder $E$. We employ a PointNet architecture \cite{} for the encoder $E$, and the final output of encoder is denoted as $G_e = E(G_m)$. 


% \ca{better use paragraph.}
\paragraph{Embedding Network.}
\label{sec.embedding-network}
We utilize an embedding network with an architecture similar to PointNet \cite{pointnet++} to embed the watermark message into the 3DGS.
% due to its ability to effectively capture local features and fine detail of the 3D models. 
Specifically, we begin by normalizing the center position $M_{tex}$, scaling factor $S_{tex}$, rotation $R_{tex}$, opacity $A_{tex}$ and color $C_{tex}$ of the textured 3DGS $G_{tex}$ into a range of $[-1, 1]$. 
% This normalization is crucial due to the significant disparities in the values of these Gaussian attributes. 
Then, we concatenate all normalized Gaussian attributes into a tensor $G_t \in \mathbb{R}^{(N+N_r)\times d_g}$, where $d_g = 3 + 3 + 4 + 1 + 3\times (k+1)^2$. Next, we replicate each bit of the message $N + N_r$ times and concatenated it with the $G_t$ to produce a feature tensor $G_m \in \mathbb{R}^{(N + N_r) \times (d_g + l_b)}$, which serves as the input for the embedding network. The network processes $G_m$ with multiple cascaded blocks. Each block groups the input Gaussian primitives into local regions based on the center position. The point features of the primitives within the same region are aggregated with a pooling layer and subsequently processed through a MLP layer, resulting the output of the block. The output of the embedding network, denoted as $G_{out} \in \mathbb{R}^{(N+N_r)\times d_g}$, is interpreted as the residual of $G_{tex}$. We project $G_{out}$ onto the range $[-1, 1]$ and split it into Gaussian attributes $(M_{res}, S_{res}, R_{res}, C_{res}, A_{res})$. These attributes are added to $G_{tex}$ to produce the final watermarked Gaussian splatting $G_{wm}(M_{wm}, S_{wm}, R_{wm}, C_{wm}, A_{wm})$. This process is formulated as follow:
\begin{equation}
\begin{split}
    &G_{out} = E(G_m) \\
    &G_{out} = \text{Tanh}(G_{out}) \times 2 - 1 \\
    &M_{res}, S_{res}, R_{res}, C_{res}, A_{res} = \text{Split}(G_{out}) \\
    &M_{wm} = M_{tex} + s_\mu M_{res} \\
    &S_{wm} = S_{tex} + s_s S_{res} \\
    &R_{wm} = R_{tex} + s_r R_{res} \\
    &C_{wm} = C_{tex} + s_c C_{res} \\
    &A_{wm} = A_{tex} + s_\alpha A_{res} \\
\end{split}
\label{PointNet}
\end{equation}
where $E$ represents the embedding network. The parameter $s_\mu$, $s_s$, $s_r$, $s_c$, and $s_\alpha$ denotes the rescale factor. In practice, the number of blocks in our embedding network is set to $2$, and the hidden dimension is set to $64$, enabling effective and efficient embedding. 
\ca{simplify and shorten.}

\paragraph{Distortion layer.}
\label{sec.method_distortion_layer}
To enhance the robustness of our framework against various distortions, we incorporate a distortion layer that intentionally degrades the rendered images of the watermarked 3DGS. This layer incorporates several commonly used distortions, including dropout, crop, and JPEG compression. Specifically, assume that the rendered image of the input and watermarked 3DGS under camera pose $v$ is denoted as $I_{in} = R(G_{in}, v)$ and $I_{wm}=R(G_{wm}, v)$ representatively, where $R$ represents the differentiable tile rasterizer \cite{3dgs}. Within the distortion later, dropout operations replace pixels of $I_{wm}$ with corresponding regions from $I_{in}$. Crop operation introduces a random square crop on the rendered image $I_{wm}$, and JPEG compression apply JPEG drop and JPEG mask on the $I_{wm}$. These operations, along with an identity operation that outputs $I_{wm}$ without unaltered, are sampled uniformly to produce the distorted image $I_{wm}'$. As all these distortions are differentiable, our network can be trained in an end-to-end manner.
% 1) additive Gaussian noise applied on the attributions of the Gaussian primitives; 2) random scaling of the Gaussian splatting with a scaling factor $s$; 3) random cropping of the Gaussian primitives. \cref{fig:pipeline} demonstrates images rendered by 3DGS with and without the introduced distortion. As all these distortions are differentiable, our network can be trained in an end-to-end manner.

\paragraph{2D Watermark Decoder}
\label{sec.method_2D_decoder}
We employ a 2D decoder to recover the embedded message from the distorted rendered image $I_{wm}'$. Specifically, we utilize the HiDDeN decoder \cite{hidden} as our 2D decoder due to its widely application. The decoder employs multiple 2D convolution layers to extract features from the rendered image $I_{wm}'$, followed by a global spatial pooling to produce the predicted message $M_{pred}$. 
% we utilize a CNN-based neural network as the 2D decoder. 
% we utilize differentiable tile rasterization method \cite{} to render images from Gaussian splatting $G_{wm}$. Subsequently, 
% a CNN-based neural network is employed to extract the message from the rendered images. 
% The architecture of the CNN network follows that of the HiDDeN decoder \cite{hidden}, where multiple 2D convolution layers are employed to extract features from the rendered image $I$, followed by a global spatial pooling to produce the predicted message $M_{pred}$. 
% This process can be formulated as follows:
% \begin{equation}
%     M_{pred} = D(I_{wm}')
%     \label{decoder}
% \end{equation}
To improve the accuracy of the 2D decoder, we pre-train the HiDDeN model on a dataset consisting of the render images generated from input 3DGS. The pre-trained HiDDeN decoder is then used to initialize our 2D decoder. Subsequently, we jointly train our 3D encoder and 2D decoder to optimize the overall performance of the watermarking framework.

% \subsection{Optimization}
% \label{sec.method_loss_funs}
\subsection{Loss Function}
The total loss used during the training process is a weighted sum of the image loss $\mathcal{L}_{img}$ and message loss $\mathcal{L}_{msg}$:
\begin{equation}
    \mathcal{L} = W_{img}\mathcal{L}_{img} + W_{msg}\mathcal{L}_{msg}
    \label{loss}
\end{equation}

To ensure that the watermarked 3DGS closely resembles the input 3DGS, we employ the distance between the images rendered from the input and watermarked 3DGS as supervision. Specifically, we apply both the mean square error (MSE) loss and the LPIPS \cite{lpips} loss, formulated as follows:
\begin{equation}
\begin{split}
    \mathcal{L}_{img} = \mathcal{L}_{MSE}(R(G_{in}, v), R(G_{wm}, v)) + \\
    \mathcal{L}_{LPIPS}(R(G_{in}, v), R(G_{wm}, v))
\end{split}    
\label{img loss}
\end{equation}
Additionally, we use the difference between input message $M$ and extracted message $M_{pred}$ to supervise our model, which is expressed as:
\begin{equation}
    \mathcal{L}_{msg} = \mathcal{L}_{MSE}(M, M_{pred})
    \label{msg loss}
\end{equation}

% When calculating the training loss, the camera pose $v$ is sampled randomly, where the elevation, azimuth are uniformly sampled from interval $[-90, 90]$ and $[0, 360]$, respectively. 
% In the training process, we optimize both the encoder and decoder in an end-to-end manner using the proposed loss function. 

% \paragraph{Adaptive weighting.}
% \ca{add weighting stretagy}

% \subsection{Implement Detail}
% \subsection{Dataset}
% \label{sec.method_dataset}



% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
%     \hline
%           $s_\mu$ & $s_s$ & $s_r$ & $s_c$ & $s_\alpha$ & $w_s$ & $w_\alpha$ \\
%     \hline
%           0.2 & 2 & 0.5 & 8 & 8 & 0.5 & 1 \\
%     \hline
%     \end{tabular}
%     \caption{Hyperparameter setting.}
%     \label{tab:hyperparameter}
% \end{table}


==> sec/_4_experiments.tex <==
\section{Experiments}
\label{sec.exps}
\subsection{Experimental Setting}
\paragraph{Dataset.}
To validate the generalizability of our method, we use datasets from both the source domain (for training and testing) and the target domain (for testing only).


\begin{itemize}
    \item For the \textbf{source domain}, we adopt the widely used Objaverse dataset \cite{objaverse}.
Specifically, we randomly sampled 1500 objects. For each object, we render 80 views using the official rendering scripts \cite{objaverse}.
We then optimize the original 3DGS using these rendered views with the official Gaussian splatting codebase \cite{3dgs}, forming the Objaverse$^{GS}_{train}$ dataset.
In addition, we sample another 100 objects from Objaverse to create a source-domain test set, ObjaverseGS$^{GS}_{test}$.

\item For the \textbf{target domain}, we follow standard practice in object-based 3DGS studies, and employ the Blender \cite{nerf} and OmniObject3D \cite{wu2023omniobject3d} datasets for further evaluation. Since initializing the original 3DGS is resource-intensive, we randomly sample 100 objects from OmniObject3D and construct original 3DGS to form a test set, Omniobject3D$^{GS}$. For Blender, we use all objects to form a test set, Blender$^{GS}$. 
\end{itemize}




% Following most existing studies on 3DGS, we utilize the Blender and OmniObject3D dataset \cite{nerf} for validation. To validate the model generalization, we also evaluate our model on the OmniObject3D \cite{wu2023omniobject3d} dataset. The OmniObject3D dataset consists of over 6,000 objects, and we randomly sample 100 objects from the OmniObject3D dataset as the test dataset. We compare the proposed WaterGS framework with other 3D watermarking methods on the Blender dataset, the OmniObject3D dataset, and our constructed 3DGS dataset.

\paragraph{Metrics.} The performance of our method is evaluated in terms of both the visual quality and data capacity. For visual quality, we evaluate the PSNR, SSIM, and LPIPS \cite{lpips} between the images rendered by the original and watermarked 3DGS. For data capacity, we calculate the bit accuracy of the extracted message from images rendered from watermarked 3DGS under various lengths of message $N_b \in \{4, 8, 16, 32, 64, 128\}$. In all experiments, we evaluate our methods as well as the baseline in our 3DGS test dataset with 100 objects. For each object in the test dataset, we uniformly sample 40 camera poses around the input 3D object to calculate the evaluation matrices. These camera poses used in the evaluation process have elevation sampled uniformly from $[-5^\circ, 5^\circ]$ and azimuth with value $9^\circ \times r, r\in [0, 39]$.  

\paragraph{Implementation details.}
% the embedding network has two PointNet layer with hidden dimension of 64, while the decoder follows the same architecture of the HiDDeN decoder \cite{} as menthoned in \cref{sec.method_2D_decoder}. 
% the learnable weights in \cref{split_GS} are initialized to $w_s=0.5$ and $w_\alpha=10$. 

% $0.014$, $0.5$, $0.1$, $1.0$, and $1.0$. 
% During the Markers generation process, the radio $p_s$ of randomly sampled Gaussian primitives to the input Gaussian primitives is set to $0.2$, and the split times $N_{split}$ is set to $2$. 
% The hyperparameters in \cref{PointNet} are set as $s_\mu=0.1$, $s_s=0.5$, $s_r=0.5$, $s_c=4$, and $s_\alpha=8$. 
The training is conducted on 8 NVIDIA Tesla V100 GPUs.
We first pre-train the HiDDeN \cite{hidden} model on $20,000$ sampled images from the rendered images of the Objaverse dataset and utilize the pretrained HiDDeN decoder to initialize our 2D decoder.
For training \ours, we utilize the Adam optimizer with a learning rate $1\times 10^{-4}$ for both the encoder and decoder. Due to the varying number of Gaussian primitives across different 3DGS models, the batch size is set to 1 in the training. In each iteration, images are rendered from 4 randomly sampled camera poses for both the watermarked and input 3DGS, with the elevation and azimuth of the camera poses sampled from the intervals $[-90^\circ, 90^\circ]$ and $[0^\circ, 360^\circ]$, respectively. The models are trained for $800,000$ iterations. We divide the training into three stages to implement our adaptive weighting strategy. The first stage spans from iteration $0$ to $200,000$, the second from iteration $200,000$ to $500,000$, and the final stage from iteration $500,000$ to $800,000$. Initially, the training is conducted without applying any distortion. Upon completion of the three training stages, we add the distortion layer and continue training for an additional $400,000$ iterations. Our experiments are conducted on message length $l_b=16$ unless mentioned specifically.

The learnable perturbation amplitude $\omega_j$ for Gaussian properties are initialized as follows: position at 0.01, scaling at 0.5, rotation at 0.1, and both opacity and color at 1.0. The selection ratio $\gamma$ is chosen as 0.4 and will be examined in detail in \cref{sec:ablation}.


% \ca{revise}

% To ensure better coverage during training, the model is designed to first learn to embed the watermark message and subsequently enhance the visual quality of watermarked Gaussian splatting. Consequently, the initial weight of the message loss $W_{msg}$ is set to a relatively large value of $80$, and is linearly decreased to 1 throughout the first $200,000$ iterations. In contract, the weight of the image loss $W_{img}$ is initialized to 0, and is linearly increased to $1$ over the same $200,000$ iterations. Furthermore, to improve the visual quality further, the weight of image loss $W_{img}$ is linearly increase from $1$ to $2$ during the iteration range from $500,000$ to $600,000$.

% \paragraph{Baseline.} As there are currently no watermarking algorithms specifically designed for 3D Gaussian splatting, we compare our method against existing 2D and 3D watermarking strategies that can be applied to 3D Gaussian splatting. 
% % Specifically, we design three baseline: \textbf{HiDDeN\cite{} + 3D Gaussian splatting}, \textbf{CopyRNeRF\cite{} + 3D Gaussian splatting}, and \textbf{WaterRF\cite{} + 3D Gaussian splatting}. 
% For the 2D watermarking strategy, we incorporate the HiDDeN model into 3D Gaussian splatting, resulting in the baseline method denoted as \textbf{HiDDeN\cite{} +3DGS}. In this baseline method, we employ the HiDDeN model to watermark the training images and subsequently optimize the 3D Gaussian splatting using these watermarked images. To establish this baseline, we pre-trained the HiDDeN models on 20,000 sampled images from the Gobjaverse dataset, adhering to the same configuration utilized for the pre-training of our 2D decoder. For the 3D watermarking strategy, we apply CopyRNeRF \cite{} and WaterRF \cite{} on 3D Gaussian splatting. Specifically, CopyRNeRF proposes substituting the original color representation in NeRF with a watermark-embedded color representation. Accordingly, in our baseline method termed \textbf{CopyRNeRF + 3DGS}, we fuse the watermark message into the color attribution of the input Gaussian splatting using a MLP. Similarly, WaterRF\cite{} proposes fine-tuning NeRF to embed watermark messages into the rendered images, with a discrete wavelet transform (DWT) applied to the rendered images for extracting the embedded messages. For the baseline method \textbf{WaterRF\cite{} + 3DGS}, we modify the WaterRF pipeline by replacing the 3D model represnted by NeRF with the 3D Gaussian splatting model, maintaining the original WaterRF framework for message embedding and extraction.

% Specifically, our baseline methods include: 1) \textbf{HiDDeN\cite{} + 3D Gaussian splatting}: watermarking the training images with HiDDeN prior to their utilization in optimizing the 3D Gaussian splatting; 2) \textbf{CopyRNeRF\cite{} + 3D Gaussian splatting}: . 

\paragraph{Baseline.} Given the absence of generalizable watermarking approaches for 3DGS, we compare our method against existing 2D and optimization-based 3D watermarking strategies.
For the 2D watermarking strategy, we incorporate the HiDDeN model \cite{hidden} with 3DGS, hereafter referred to as \textbf{HiDDeN + 3DGS}. In this baseline, the HiDDeN model is utilized to watermark the training images, which are then used to optimize the 3DGS. We pre-train the HiDDeN models using the same configuration as that employed for the pre-training of our 2D decoder.
For 3D representation, we select the state-of-the-art published works, \textbf{WateRF} \cite{waterf} for NeRF, and \textbf{GaussianMarker} \cite{NEURIPS2024_39cee562} for 3DGS. The mesh-based method \cite{mesh_watermark1} is excluded due to the significant differences in encoding and rendering compared to 3DGS, and the lack of open-source code.


% For the 3D watermarking strategy, we adopt \textbf{WateRF}  \cite{waterf} designed for NeRF and \textbf{GaussianMarker} \cite{NEURIPS2024_39cee562} designed for 3DGS as baseline. For implement WateRF on the Objaverse and OmniOnject3D dataset, we first apply the Tensorf \cite{tensorf} method to the rendered images from these datasets to generate the corresponding NeRF models. Subsequently, we apply the WateRF to the generated NeRF models for the comparison experiments.
% For the 3D watermarking strategy, we adopt \textbf{WateRF} \cite{waterf} as the baseline, which is specifically designed for watermarking NeRF representation. In our experimental setup, we first apply the Tensorf \cite{tensorf} method to the rendered images from our 3DGS test datasets to generate the corresponding NeRF models. Subsequently, we apply the WateRF to the generated NeRF models for the comparison experiments.


\subsection{Main Results}
% \ca{highlight why small training data still work.}
% \subsection{Compare with Baseline}
\paragraph{Quantitative comparison.}
We quantitatively compare our framework with all baseline methods on both the source domain (Objaverse$^{GS}_{test}$) and target domain (Blender$^{GS}$, Omni3DObject$^{GS}$) datasets, evaluated on an A100 GPU. The results are presented in \cref{tab:comparison}.
Note that our trained model is not fine-tuned on the target domain datasets, Blender$^{GS}$, Omni3DObject$^{GS}$, underscoring the model's adaptability.
The experimental results demonstrate that our method achieves admirable results on all test datasets, which demonstrates the generalization of our method. In addition, our method achieves better performance than  the NeRF watermarking methods. For the optimization-based 3DGS watermarking method GaussianMarker, although the accuracy of our method is slightly lower than that in the target domain, our method achieves much better visual quality. More importantly, we compute the average watermark embedding time of the test dataset, our method requires significantly less time to embed the messages compared with all the other methods, highlighting the efficiency of our method. 

% The experimental results demonstrate that the embedding time of the WaterGS is significantly lower than other baseline methods.

% \paragraph{Qualitative comparison.}
% \ca{add}

\begin{table*}[ht!]
\centering
\caption{Quantitative comparison. ``E-time'' is short for average watermark embeddding time tested on an A100 GPU. 
The best values are highlighted in \textbf{bold}, while the second-best accuracy and PSNR are indicated with an \underline{underline}. Note that WateRF and GaussianMarker are iterative optimization-based methods.
}
\label{tab:comparison}
\resizebox{\textwidth}{!}{  % This ensures the table fits within the page width
\begin{tabular}{l ccccc ccccc ccccc}
\toprule
\multirow{2}{*}{\textbf{Method}}  
& \multicolumn{5}{c}{\textbf{Objaverse$^{GS}_{test}$ (Source domain)}} 
& \multicolumn{5}{c}{\textbf{Blender$^{GS}$ (Target domain)}} 
& \multicolumn{5}{c}{\textbf{Omni3DObject$^{GS}$ (Target domain)}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
& E-time (s)$\downarrow$ & Acc$\uparrow$ & PSNR$\uparrow$& SSIM$\uparrow$  & LPIPS$\downarrow$ 
& E-time (s)$\downarrow$ & Acc$\uparrow$ & PSNR$\uparrow$& SSIM$\uparrow$  & LPIPS$\downarrow$ 
& E-time (s)$\downarrow$ & Acc$\uparrow$ & PSNR$\uparrow$& SSIM$\uparrow$  & LPIPS$\downarrow$\\
\midrule
Hidden \cite{hidden}+3DGS & 260 & 52.88 & 29.71 & 0.9769 & 0.0459
& 350 & 49.99 & 14.53 & 0.7440 & 0.3671
& 300 & 50.0 & 17.06 & 0.8344 & 0.2889 \\

WateRF \cite{waterf} & 4400 & 83.43 & 33.07 & 0.9626 & 0.0259 
& 4900 & 93.26 & 30.81 & 0.9472 & 0.0577 
& 6000 & 79.54 & 31.16 &  0.9211 & 0.0978 \\

GaussianMarker \cite{NEURIPS2024_39cee562} & 580 & \underline{90.69} & \textbf{35.53} & 0.9760 & 0.0281 
& 340 & \textbf{98.32} & 28.37 & 0.9295 & 0.0516
& 290 & \textbf{94.07} & 31.56 & 0.9413 & 0.0643 \\

\ours~(ours) & \textbf{0.11} & \textbf{95.46} & \underline{34.86}& \textbf{0.9837} & \textbf{0.0249}
& \textbf{0.33} & \underline{93.56} & \textbf{33.40} & \textbf{0.9828} & \textbf{0.0154}
& 0.04& \underline{93.63} & \textbf{37.59} & \textbf{0.9743} & \textbf{0.0229} \\
\bottomrule
\end{tabular}
}
\end{table*}

\paragraph{Qualitative comparison.}
% \ca{add}
% To further verify the visual quality of our method, we calculate the differences between images rendered from the input and watermarked 3DGS on the 3DGS test dataset built on Gobjaverse dataset and the Blender dataset. 
The qualitative comparison is illustrated in  \cref{fig:comparison_baseline} and \cref{fig:comparison_blender}. 
% The discrepancies between input and watermarked 3DGS of our method are minimal, indicating that our method embeds watermark messages with negligible impact on the visual quality. For the baseline {HiDDeN + 3DGS}, we observe that the background of the rendered image is filled with large Gaussian primitives with dark color. The issue may be attributed to the use of the HiDDeN encoder to the training images of 3DGS, which introduces invisible noise into the image background. The 3DGS optimization process attempts to fit these noises to learn the embedded watermark message, resulting in the appearance of large Gaussian primitives. In the case of the baseline {WateRF}, while it achieves good bit accuracy, the surfaces of watermarked objects exhibit significant artifacts, leading to a reduction in visual quality.
The discrepancies between the input and watermarked 3DGS in our method are minimal, indicating that watermark messages are embedded with negligible impact on visual fidelity. By contrast, the {HiDDeN + 3DGS} baseline exhibits large, dark Gaussian primitives in the background of rendered images. This effect arises from using HiDDeN’s encoder on the 3DGS training images, which injects invisible noise into the image background. The 3DGS optimization process then attempts to fit these background noises to learn the watermark message, ultimately producing conspicuous Gaussian artifacts.

Meanwhile, WateRF achieves good bit accuracy but introduces noticeable artifacts on the surfaces of watermarked objects, reducing overall visual quality. These results highlight the superior balance our method strikes between embedding robustness and visual realism.

\if false
\begin{table*}[ht!]
\centering
\caption{caption}
\label{tab:comparison}
\begin{tabular}{lccccccccccc}
\toprule
\multirow{2}{*}{Method} 
& \multicolumn{5}{c}{ObjaverseGS$_{test}$} 
& \multicolumn{5}{c}{BlenderGS} 
& \multicolumn{5}{c}{Omni3DObjectGS} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}\cmidrule(lr){12-16}
& E-time (s) & Acc (\%) & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
& E-time (s) & Acc (\%) & PSNR$\uparrow$ & LPIPS$\uparrow$ & SSIM$\downarrow$
& E-time (s) & Acc (\%) & PSNR$\uparrow$ & LPIPS$\uparrow$ & SSIM$\downarrow$ \\
\midrule
HiDDeN+3DGS
& 1 & 1 & 22.64 & 0.21 & 0.75 
& 19.43 & 0.39 & 0.56 
& 22.49 & 0.49 & 0.60 \\
WateRF
& 23.54 & 0.13 & 0.90 
& 19.80 & 0.30 & 0.62 
& 23.27 & 0.48 & 0.69 \\
GaussianMarker
& 23.46 & 0.20 & 0.86 
& 19.70 & 0.26 & 0.60 
& 26.33 & 0.38 & 0.70 \\
\ours
& 22.42 & 0.17 & 0.80 
& 20.54 & 0.24 & 0.64 
& 23.19 & 0.47 & 0.66 \\
\bottomrule
\end{tabular}
\end{table*}
\fi

% \begin{table}[htbp]
%     \begin{center}
%     \setlength{\tabcolsep}{2.5pt}
%     \resizebox{0.96\linewidth}{!}{
%     \begin{tabular}{cccccc}
%     \toprule[1pt]
%      & Emb. Time (s) & Acc (\%)$\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
%     \hline
%     \multicolumn{6}{c}{\textbf{\textit{Blender Dataset}}} \\
%     GaussianMarker & 0.34K & \textbf{98.32} & 28.37 & 0.9295 & 0.0516 \\
%     % \hline
%     CopyRNeRF & 2,048K & 91.59 & 31.56 & 0.9811 & 0.02853 \\
%     % \hline
%     StegaNeRF & 3K  & 93.09 & 31.64 & 0.9573 & 0.0262 \\
%     % \hline
%     WateRF & 5K & 93.26 & 30.81 & 0.9472 & 0.0577 \\
%     % \hline
%     Ours & \textbf{0.3306} & 93.56 & \textbf{33.40} & \textbf{0.9828} & \textbf{0.0154} \\
%     \toprule[1pt]
%     \multicolumn{6}{c}{\textbf{\textit{OmniObject3D Dataset}}} \\
%     GaussianMarker & 0.30K & 96.63 & 30.08 & 0.9353 & 0.0796 \\
%     % \hline
%     WateRF  \\
%     % \hline
%     Ours & 0.0421& 93.63 & 37.59 & 0.9743 & 0.0229 \\
%     \toprule[1pt]
%     \multicolumn{6}{c}{\textbf{\textit{Objaverse Dataset}}} \\
%     GaussianMarker  \\    % \hline
%     % \hline
%     WateRF & 4K & 83.43 & 33.07 & 0.9626 & 0.0259 \\
%     % \hline
%     Ours & 0.1101 & 93.56 & \textbf{33.40} & \textbf{0.9828} & \textbf{0.0154} \\
%     \toprule[1pt]
    
%     \end{tabular}
%     }
%     \end{center}
%     \vspace{-20pt}
%     \caption{Comparison on various dataset with 16 bits messages.
%     The embedding time (s) is tested on one A100 GPU. We randomly select 100 object from the Objaverse dataset and OmniObject3D dataset for evalution. 
%     \ca{note generalizable or not.}
%     % , bit accuracy ($\%$), and visual qualities of our method compared with other existed methods on the Blender dataset.
%     }
%     % \ca{identify generalizable or not. cite} 
% \vspace{-10pt}
% \label{tab.blender1}
% \end{table}

% \begin{table}[htbp]
%     \begin{center}
%     \setlength{\tabcolsep}{2.5pt}
%     \resizebox{0.96\linewidth}{!}{
%     \begin{tabular}{cccccc}
%     \toprule[1pt]
%      & Emb. Time (s) & Acc (\%)$\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
%     \hline
%     GaussianMarker \\
%     \hline
%     StegaNeRF \\
%     \hline
%     WateRF \\
%     \hline
%     Ours  \\
%     \toprule[1pt]
%     \end{tabular}
%     }
%     \end{center}
%     \vspace{-20pt}
%     \caption{Comparison on the OmniObject3D dataset with 16 bits messages.
%     The embedding time (s) is tested on one A100 GPU. 
%     \ca{note generalizable or not.}
%     % , bit accuracy ($\%$), and visual qualities of our method compared with other existed methods on the Blender dataset.
%     }
%     % \ca{identify generalizable or not. cite} 
% \vspace{-10pt}
% \label{tab.omni3d}
% \end{table}

% % \if false
% \begin{table}
%     \begin{center}
%     \setlength{\tabcolsep}{2.5pt}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{cccccc}
%     % \begin{tabularx}{\textwidth}{XXXXX}
%     % \begin{tabular}{p{2.2cm}p{1.3cm}p{1.1cm}p{1.1cm}p{1.1cm}}
%     \toprule[1pt]
%      & Emb Time & Acc $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
%     \hline
%     \makecell{HiDDeN \cite{hidden} + 3DGS} & 263.5 & 52.88 & 29.71 & 0.9769 & 0.0459 \\
%     \hline
%     % \makecell{CopyRNeRF + 3DGS} & 43.75 & 38.48 & 0.9865 & 0.0289 \\
%     % \hline
%     \makecell{WateRF \cite{waterf}} & 4380 & 83.43 & 33.07 & 0.9626 & 0.0259 \\
%     \hline
%     Ours & 0.1101 & 96.07 & 38.36 & 0.9898 & 0.0149 \\
%     \toprule[1pt]
%     \end{tabular}
%     }
%     \end{center}
%     \vspace{-6pt}
%     \caption{The watermark embedding time (s), bit accuracy ($\%$), and visual qualities of our method compared with baseline methods on our constructed 3DGS dataset.}
%     % \ca{identify generalizable or not. cite}
% % \vspace{-8pt}
% \label{tab.comparison_exps}
% \end{table}


\begin{figure*}
  \centering
   \includegraphics[width=0.99\linewidth]{Figs/result_4_1_v3.pdf}
   % \vspace{-8pt}
   \caption{Qualitative comparisons between our method and the baseline. We show the differences (×10) between the images rendered by the input and watermarked 3DGS. Our method achieves better PSNR and bit accuracy than baseline.}
  \label{fig:comparison_baseline}
\end{figure*}
% \vspace{-4pt}

\begin{figure*}[ht]
  \centering
  % Left side: Three horizontally arranged subfigures
  \begin{minipage}{0.73\textwidth}  % Ensures left block takes 73% of width
    \centering
    \includegraphics[width=0.32\linewidth]{Figs/MessageLoss.pdf} \hfill%
    \includegraphics[width=0.32\linewidth]{Figs/ImageLoss.pdf} \hfill%
    \includegraphics[width=0.32\linewidth]{Figs/TotalLoss.pdf}
    \caption{
      The evolution of watermark, rendering, and total loss during training under different settings. ``AMC-F'' and ``AMC-L'' denote different settings. Ours ``AMC-L'' best balances the losses.
    }
    \label{fig:training_loss}
  \end{minipage}%
  \hfill%
  % Right side: Single independent figure
  \begin{minipage}{0.243\textwidth}  % Ensures right block takes 26% of width
    \centering
    \includegraphics[width=\linewidth]{Figs/lb_vs_acc_psnr.pdf}
    \caption{The model performance under various message lengths $l_b$.}
    \label{fig:ablation_studies}
  \end{minipage}
  \vspace{-8pt}
\end{figure*}
% \vspace{-10pt}

\begin{figure}
  \centering
   \includegraphics[width=0.99\linewidth]{Figs/comparison_blender_v1.pdf}
   \vspace{-8pt}
   \caption{Qualitative comparisons between our method and WateRF \cite{waterf} on the Blender dataset \cite{nerf}. Our method achieves better visual quality than WateRF.}
  \label{fig:comparison_blender}
\end{figure}
% \vspace{-4pt}
% \ca{the first case is not good, 3) better no cropping}}

\begin{figure}
  \centering
   \includegraphics[width=0.99\linewidth]{Figs/result_4_2_v5.pdf}
   \caption{Qualitative comparisons between our method with and without Adaptive Marker Control (AMC). Without AMC, artifacts appear on the rendered images. }
   % \ca{1) more views, 2) render only markers}
  \label{fig:ablation_noise}
  % \vspace{-40pt}
\end{figure}

\subsection{Ablation Study}
\label{sec:ablation}
% \ca{
% 1. marker ratio
% 2. learnable weight
% 3. decoder
% 4. bits length, embedding capacity (can move to an independent part)
% }
% \paragraph{Ablation on Markers.}
% \subsubsection{Ablation on Markers.}
% We analyze the impact of the W-Marker introduced in \cref{sec.W-Marker} on the performance of our WaterGS framework. We conducted the experiments on different super-parameter setting of random Gaussian primitives, and the results are presented in \cref{tab.ablation_noise}.

% In contrast, these artifacts are effectively mitigated when the random Gaussian primitives are incorporated, leading to a higher fidelity in the rendered images. Thus, the inclusion of random Gaussian primitives proves to be essential for maintaining the visual integrity of our watermarking framework.

% \begin{table}
%     \begin{center}
%     \setlength{\tabcolsep}{2.5pt}
%     \begin{tabular}{cc|cccc}
%     \toprule[1pt]
%      $p_s$ & $N_{split}$ & Acc ($\%$) $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
%     \midrule
%     \multicolumn{6}{c}{\textbf{\textit{Ours}}} \\
%     $0.2N$ & 2 & 96.07 & 38.36 & 0.9898 & 0.0149 \\
%     \midrule
%     \multicolumn{6}{c}{\textbf{\textit{Without Random Gaussian Primitives}}} \\
%     0 & 0 & 90.14 & 31.61 & 0.9760 & 0.0366 \\
%     \midrule
%     \multicolumn{6}{c}{\textbf{\textit{Frozen learnable weights $s_s$ and $s_\alpha$}}} \\
%     $0.2N$ & 2 & 94.96 & 31.24 &0.9667 & 0.0568 \\
%     \midrule
%     \multicolumn{6}{c}{\textbf{\textit{Ablation on $p_s$}}} \\
%     % $0.05N$ & 2 & - & - & - & - \\
%     $0.1N$ & 2 & 94.14 & 38.03 & 0.9893 & 0.0161 \\
%     $0.01N$ & 2 & 94.00 & 36.77 & 0.9892 & 0.0185 \\
%     $0.005N$ & 2 & 92.59 & 34.31 & 0.9851 & 0.0241 \\
%     \midrule
%     \multicolumn{6}{c}{\textbf{\textit{Ablation on $N_{split}$}}} \\
%     $0.2N$ & 1 & 94.80 & 39.41 & 0.9917 & 0.0119 \\
%     \midrule
%     \multicolumn{6}{c}{\textbf{\textit{Ablation on Random Color}}} \\
%     $0.2N$ & 2 & 93.93 & 39.55 &0.9909 & 0.0138 \\
    
%     \toprule[1pt]
%     \end{tabular}
%     \end{center}
%     \caption{Ablation study on Random Gaussian Primitives. All experiments are conducted on message length $l_b=16$. $N$ represents the number of Gaussian primitives in the input Gaussian splatting.
%       \ca{too messy, beter with a line figure}
%     }
%     % In experiments on our method \textbf{\textit{Without Random Gaussian Primitives}}, we remove the random Gaussian primitives and observe that the bit accuracies and visual quality drop significantly. In experiments of \textbf{\textit{Ablation on }}$p_s$ and \textbf{\textit{Ablation on}} $N_{split}$, we conduct experiments on various $p_s$ and $N_{split}$ to analyze the minimal number of random Gaussian primitives that ensure the bit accuracies and visual quality. We analyze the role of learnable weight $s_s$ and $s_\alpha$, as well as the role of random color setting on experiments of 
% \label{tab.ablation_noise}
% \end{table}

% \begin{table}
% \scalebox{0.9}{
% \centering

%     % \begin{center}
%     \setlength{\tabcolsep}{2.5pt}
%     \begin{tabular}{cc|cc|cccc}
%     \toprule[1pt]
    
%     RC & UW & $p_s$ & $N_{split}$ & Acc ($\%$) $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
%     \midrule
%     % \multicolumn{6}{c}{\textbf{\textit{Ours}}} \\
%     $\checkmark$ & $\checkmark$ & $0.2$ & 2 & 96.07 & 38.36 & 0.9898 & 0.0149 \\
%     % \midrule
%     % \multicolumn{6}{c}{\textbf{\textit{Without Random Gaussian Primitives}}} \\
%      - & - & 0 & 0 & 90.14 & 31.61 & 0.9760 & 0.0366 \\
%     % \midrule
%     % \multicolumn{6}{c}{\textbf{\textit{Frozen learnable weights $s_s$ and $s_\alpha$}}} \\
%     $\checkmark$ & $\times$ & $0.2$ & 2 & 94.96 & 31.24 &0.9667 & 0.0568 \\
%     % \midrule
%     % \multicolumn{6}{c}{\textbf{\textit{Ablation on $p_s$}}} \\
%     % $0.05N$ & 2 & - & - & - & - \\
%     $\checkmark$ & $\checkmark$ & $0.1$ & 2 & 94.14 & 38.03 & 0.9893 & 0.0161 \\
%     $\checkmark$ & $\checkmark$ & $0.01$ & 2 & 94.00 & 36.77 & 0.9892 & 0.0185 \\
%     $\checkmark$ & $\checkmark$ & $0.005$ & 2 & 92.59 & 34.31 & 0.9851 & 0.0241 \\
%     % \midrule
%     % \multicolumn{6}{c}{\textbf{\textit{Ablation on $N_{split}$}}} \\
%     $\checkmark$ & $\checkmark$ & $0.2$ & 1 & 94.80 & 39.41 & 0.9917 & 0.0119 \\
%     % \midrule
%     % \multicolumn{6}{c}{\textbf{\textit{Ablation on Random Color}}} \\
%     $\times$ & $\checkmark$ & $0.2$ & 2 & 93.93 & 39.55 &0.9909 & 0.0138 \\
    
%     \toprule[1pt]
%     \end{tabular}
%     % \end{center}
%     }
%     \caption{Ablation on the Markers. ``UW'' denotes the experiments updating the learnable weight $w_s$ and $w_\alpha$. ``RC'' denotes the experiments with Markers assigned with random colors.
%     \ca{remove}
%     }
%     % \ca{too messy, beter with a line figure}
%     % In experiments on our method \textbf{\textit{Without Random Gaussian Primitives}}, we remove the random Gaussian primitives and observe that the bit accuracies and visual quality drop significantly. In experiments of \textbf{\textit{Ablation on }}$p_s$ and \textbf{\textit{Ablation on}} $N_{split}$, we conduct experiments on various $p_s$ and $N_{split}$ to analyze the minimal number of random Gaussian primitives that ensure the bit accuracies and visual quality. We analyze the role of learnable weight $s_s$ and $s_\alpha$, as well as the role of random color setting on experiments of 
% \vspace{-6pt}
% \label{tab.ablation_noise}
% \end{table}


\paragraph{Impact of modules.}

We perform an ablation study to assess the impact of two main components: the Decoder Fine-Tuning strategy (DF) and the Adaptive Marker Control (AMC) module from \cref{sec:amc}. 
Within AMC, we also examine whether making the perturbation amplitude learnable further enhances performance. The results are summarized in \cref{tab:ablation_module}.
The first row shows that without fine-tuning the 2D decoder, both bit accuracy and visual quality degrade significantly.
Without AMC, the rendering fidelity remains high since the original 3DGS is well-optimized for rendering loss. However, the model fails to improve decoding accuracy due to being trapped in a local minimum of the rendering objective.
Introducing perturbations with fixed amplitude (AMC-F) enhances decoding accuracy while maintaining high rendering fidelity. Further allowing the perturbation amplitude to be learnable (AMC-L) results in additional gains in both accuracy and visual quality. This demonstrates that adaptive control over perturbations is crucial for balancing watermark embedding and rendering quality.

\cref{fig:training_loss} illustrates the evolution of watermark loss, rendering loss, and total loss over iterations for different settings. The without-AMC setting struggles to minimize message loss, as it gets trapped in a local minimum dictated by rendering loss. The AMC-F setting improves message loss decay but fails to optimize rendering loss effectively. In contrast, our AMC-L setting achieves the best balance between watermark accuracy and rendering fidelity, demonstrating its ability to optimize both objectives simultaneously.

The final learned perturbation amplitudes are $\omega_{color}=1.489, \omega_{opacity}=0.2103, \omega_{position}=0.0163, \omega_{scale}=9.9999e-5, \omega_{rotation}=0.0929$.
These values confirm how differentiable rendering in a 3DGS framework influences each parameter. Opacity and color affect the gradient in a nearly linear manner. Position gradients scale with distance from the Gaussian center, normalized by its spread. Scale and rotation are more sensitive, since they depend on squared distances and can dramatically impact Gaussians with small spreads. Overall, this analysis provides insight into how each property contributes to the gradient when 3DGS differentiable rendering is integrated into the learning loop.

% As indicated in the first row of \cref{tab.learnable_weight_abblation}, the exclusion of AMC leads to a noticeable degradation in bit accuracy and visual quality. In addition, \cref{fig:ablation_noise} offers a visual comparison of the rendered images produced by our method with and without AMC. As shown in \cref{fig:ablation_noise}, the absence of the AMC results in the appearance of noticeable artifacts along the texture and edge of objects, which significantly diminishes the overall visual quality. 

%  The last row of \cref{tab.learnable_weight_abblation} demonstrates that the bit accuracy of our framework without fine-tuning the decoder fails to extract the watermark message correctly. This result demonstrates that the framework can not optimize both bit accuracy and visual quality by adjusting only the 3D encoder, even though the 2D decoder has achieved high bit accuracy on 2D rendering images after pre-training.

 
% \textcolor{blue}{\paragraph{Ablation on the learnable perturbation amplitude.} We conduct an ablation study on the learnable perturbation amplitude proposed in \cref{sec:amc} to analyze its impact on the model performance. Specifically, we train the model under the following setting: 1) \textbf{\emph{AMC without learnable perturbation amplitude}}: The perturbation amplitude is fixed without update during training; 2) \textbf{\emph{AMC with partial learnable perturbation amplitude}}: Only the perturbation amplitude of Gaussian scaling and opacity is updated, and the perturbation amplitude of other Gaussian properties are fixed; 3) \textbf{\emph{AMC with learnable perturbation amplitude}}: The perturbation amplitude of all Gaussian properties are updated during training. The loss curve and evaluation results of these settings are shown in \cref{fig:training_loss} and \cref{tab.learnable_weight_abblation} respectively. We set the Marker ratio to 0.4 in these experiments. The experimental results show that the message loss and performance on the test dataset of the model with learnable perturbation amplitude is better than that without learnable amplitude, which shows that the learnable amplitude enables the model to achieve a better trade-off on the message accuracy and visual quality. Furthermore, the model with partial learnable perturbation amplitude achieves better performance than that with all amplitude learnable. This result demonstrates that the adjustment on the perturbation of Gaussian scaling and opacity is sufficient for the model to control the perturbation of Gaussian primitives, since adjusting scaling leads to the change of perturbated Gaussian primitive's size, and the opacity is relative to the visibility of perturbated Gaussian primitives. Finally, We also notice that the rendering loss of the model without learnable amplitude is slightly lower than that with learnable amplitude, but its visual quality on the test dataset is worse. This result illustrates that the learnable amplitude may be beneficial to improve the generalization. }


% % In contrast, these artifacts are effectively mitigated when the random Gaussian primitives are incorporated, leading to a higher fidelity in the rendered images. Thus, the inclusion of random Gaussian primitives proves to be essential for maintaining the visual integrity of our watermarking framework.

% \begin{figure*}
%   \centering
%    \includegraphics[width=0.99\linewidth]{Figs/result_4_2_v4.pdf}
%    \caption{Qualitative comparisons between our method with and without random Gaussian primitives (RGP). We show the differences (×10) between the images rendered by the input and watermarked Gaussian splatting. When remove random Gaussian primitives, artifacts easily appear on the rendered images. \ca{1) more views, 2) render only markers}}
%   \label{fig:ablation_noise}
% \end{figure*}

% We hypothesize that the artifacts observed in the rendered images when the Markers are removed can be attributed to the training process of the model. 
% % Prior research has proposed that the watermark message is tend to embedded into the area with high frequency of the digital property \cite{high_freq}. 
% As discussed in \cref{sec.W-Marker}, the Markers provides the input 3DGS with additional high-frequency components, allowing the 3D encoder to preferentially embed the watermark message into these primitives. When the Markers are absent, the 3D encoder is more likely to embed the watermark message into the texture and edges of objects, which leads to the emergence of visible artifacts in these regions.
% % degrade the overall visual quality of the rendered images. 
% In our framework, we multiply the scaling and opacity of the Gaussian primitives in the Markers with the learnable weight $w_s$ and $w_\alpha$. These learnable weights provide the model with the flexibility to refine the visual quality while maintaining the integrity of the embedded watermark message. As a result, the model with Markers can achieve a more optimal balance between visual quality and bit accuracy. 
% % effectively minimizing artifacts and enhancing the overall performance of the watermarking framework.

\paragraph{Ablation on Marker Ratio $\gamma$.} 
We investigate how varying the ratio $\gamma$ of selected markers for perturbation affects the model’s performance. A low $\gamma$ risks remaining stuck in local minima, yielding suboptimal accuracy and visual quality. Conversely, a high $\gamma$ excessively disturbs the 3DGS structure, which can degrade rendering quality and increase training difficulty.
As shown in \cref{fig:marker_ratio}, initially increasing $\gamma$ helps the 3DGS escape local minima, improving both bit accuracy and PSNR. However, pushing $\gamma$ too high eventually lowers visual quality despite a further gain in accuracy. The excessive perturbation disrupts the original 3DGS structure, making it difficult for the 3D encoder to maintain high-fidelity rendering. Based on these observations, a moderate perturbation ratio strikes the best balance between watermark accuracy and visual quality. We select $\gamma=0.4$ as our final setting.



\if false
\begin{table}
    \begin{center}
    \setlength{\tabcolsep}{2.5pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}
    % \begin{tabularx}{\textwidth}{XXXXX}
    % \begin{tabular}{p{2.2cm}p{1.3cm}p{1.1cm}p{1.1cm}p{1.1cm}}
    \toprule[1pt]
     Markers Ratio & Acc $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    \hline
    0.0 & 90.14 & 31.61 & 0.9760 & 0.0366 \\
    \hline
    0.01 & 94.43 & 33.18 & 0.9848 & 0.0237 \\
    \hline
    0.05 & 95.07 & 32.84 & 0.9815 & 0.0302 \\
    \hline
    0.1 & 95.46 & 34.86 & 0.9837 & 0.0249 \\
    \hline
    0.2 & 95.34 & 34.55 & 0.9768 & 0.0327 \\
    \hline
    0.4 & 97.00 & 31.40 & 0.9630 & 0.0499 \\
    \hline
    0.6 & 97.25 & 28.48 & 0.9402 & 0.0773 \\
    \hline
    0.8 & 97.89 & 25.69 & 0.9147 & 0.1114 \\
    \hline
    1.0 & 97.12 & 23.35 & 0.8859 & 0.1465 \\
    \hline
    \toprule[1pt]
    \end{tabular}
    }
    \end{center}
    % \vspace{-6pt}
    \caption{The bit accuracy ($\%$) and visual qualities of our method under various Markers Ratio.}
    % \ca{identify generalizable or not. cite}
% \vspace{-8pt}
\label{tab.marker_ratio}
\end{table}
\fi
\begin{figure}
  \centering
   \includegraphics[width=0.9\linewidth]{Figs/fig5.pdf}
   \caption{The bit accuracy (\%) and visual qualities of our method under various Markers Ratio.}
   % \ca{1) more views, 2) render only markers}
  \label{fig:marker_ratio}
  %\vspace{-10pt}
\end{figure}


\begin{table}[!t]
    \centering
    \setlength{\tabcolsep}{2.5pt} % Adjust column spacing
    \renewcommand{\arraystretch}{1.2} % Keep row height consistent
    \newcolumntype{C}{>{\centering\arraybackslash}p{0.75cm}} % Tight columns for FD, AMC
    \newcolumntype{M}{>{\centering\arraybackslash}p{1.3cm}} % Medium column for Acc
    \newcolumntype{L}{>{\centering\arraybackslash}X}        % Auto-adjusted columns for PSNR, SSIM, LPIPS
    
    \begin{tabularx}{\columnwidth}{CC|M L L L}
    \toprule[1pt]
    FD & AMC & Acc $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    \midrule
    \ding{55} &               & 52.86  & 21.93  & 0.9342 & 0.0914 \\
              & \ding{55}             & 90.14  & \textbf{31.61} & \textbf{0.9760} & \textbf{0.0366} \\
              & F     & 94.96  & 31.24  & 0.9667 & 0.0568 \\
              & L             & \textbf{96.68} & 31.55 & 0.9643 & 0.0484 \\
    \bottomrule[1pt]
    \end{tabularx}
    \vspace{-6pt}
    \caption{Impact on modules. 
``FD" and ``AMC" represent ``fine-tuning decoder" and ``adaptive marker control," respectively. In the AMC column, ``F" indicates a fixed perturbation amplitude, while ``L" denotes a learnable perturbation amplitude.
    }
    \label{tab:ablation_module}
\end{table}

% \begin{table}
%     \centering
%     % Scale the table to 0.8 of the text width
%     \resizebox{0.8\textwidth}{!}{%
%         \begin{tabularx}{\columnwidth}{CC|M L L L}
%             \toprule[1pt]
%             FD & AMC & Acc $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
%             \midrule
%             \ding{55} &               & 52.86  & 21.93  & 0.9342 & 0.0914 \\
%                       & \ding{55}     & 90.14  & \textbf{31.61} & \textbf{0.9760} & \textbf{0.0366} \\
%                       & F             & 94.96  & 31.24  & 0.9667 & 0.0568 \\
%                       & L             & \textbf{96.68} & 31.55 & 0.9643 & 0.0484 \\
%             \bottomrule[1pt]
%         \end{tabularx}
%     } % end of resizebox
%     \vspace{-6pt}
%     \caption{Impact on modules. 
%     ``FD" and ``AMC" represent ``fine-tuning decoder" and ``adaptive marker control," respectively. 
%     In the AMC column, ``F" indicates a fixed perturbation amplitude, while ``L" denotes a learnable perturbation amplitude.
%     }
%     \label{tab:ablation_module}
% \end{table}



% \begin{figure}
%   \centering
%    \includegraphics[width=0.99\linewidth]{Figs/Training_Loss.pdf}
%    \vspace{-8pt}
%    \caption{Training loss of the models under various setting. ``Fix'', ``PLA'', and ``LA'' denote three types of learnable perturbation amplitude settings: fix amplitude, partial learnable amplitude, learnable amplitude. }
%   \label{fig:training_loss}
% \end{figure}
% \vspace{-4pt}


% \paragraph{Frozen on learnable weights $w_s$ and $w_\alpha$ in Markers.} We froze the values of $w_s$ and $w_\alpha$ to their initial value without updating them to analyze the role of learnable weights. As demonstrated in \cref{tab.ablation_noise}, when $w_s$ and $w_\alpha$ are frozen, the visual quality of the model drops significantly. These experimental results support our hypothesis that the model can achieve an optimal trade-off between bit accuracy and visual quality by adjusting the scaling and opacity of the Markers. When the learnable weight $w_s$ and $w_\alpha$ are fixed, the model performance declines.

% \paragraph{Ablation on $p_s$ and $N_{split}$ for Markers.} We conduct experiments on various values of $p_s$ and $N_{split}$ to analyze how model performance varies with changes in the number of random Gaussian primitives. \cref{tab.ablation_noise} demonstrates that the model performance decreases when $p_s$ is reduced. In addition, reducing $N_{split}$ from $2$ to $1$ also lead to a degradation in bit accuracy. These results indicate that reducing the number of random Gaussian primitives in the Markers, either by decreasing $p_s$ or $N_{split}$, can lead to a drop in model performance. Furthermore, even when $p_s$ reduce to a low value of $0.005$, our framework achieves better performance compared to the model without Markers, highlighting the significant role of the proposed W-Makers.

% \paragraph{Ablation on $p_s$ and $N_{split}$ for Markers.} We conduct experiments on various values of $p_s$ and $N_{split}$ to analyze how model performance varies with changes in the number of random Gaussian primitives. \cref{tab.ablation_noise} demonstrates that the model performance decreases when $p_s$ and $N_{split}$ is reduced. These results indicate that reducing the number of random Gaussian primitives in the Markers leads to a drop in model performance. Additionally, even when $p_s$ reduce to a low value of $0.005$, our framework achieves better performance compared to the model without Markers, highlighting the significant role of the proposed Markers.
% When $N_{split}=2$ and $p_s$ reduce to $0.005$, the model performance is similar as that without random Gaussian primitives. Therefore, in order to ensure better bit accuracy and visual quality, the number of Gaussian should be set to larger than $0.005N\times 2=0.01N$. 

% \paragraph{Ablation on color assignment in Markers.} We perform an ablation study on the color assignment strategy of the Markers. In this experiment, we set the color of primitives in the Markers to closely match the corresponding primitives in the input 3DGS with only a slight random variations. \cref{tab.ablation_noise} demonstrates that the bit accuracy decreases when the colors of the Markers is not set randomly. The reason may be that the Markers without random color does not provide sufficient texture to the input 3DGS, leading to a reduction in bit accuracy.


% \begin{table}
%     \begin{center}
%     \setlength{\tabcolsep}{2.5pt}
%     \begin{tabular}{cc|cccc}
%     \toprule[1pt]
%     Pretraining & NI & Acc ($\%$) $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
%     \hline
%     $\checkmark$ & $\checkmark$ & 96.07 & 38.36 & 0.9898 & 0.0149 \\
%     % \hline
%     $\times$ & $\checkmark$ & 83.84 & 37.57 & 0.9893 & 0.0185 \\
%     % \hline
%     $\checkmark$ & $\times$ & 95.88 & 37.89 & 0.9899 & 0.0169 \\
%     \toprule[1pt]
%     \end{tabular}
%     \end{center}
%     \caption{Ablation on the pre-training decoder and input normalization (NI) strategy utilized in the embedding process. The experiments are conducted on message length $l_b=16$.}
% \label{tab.ablation_decoder_and_normin}
% \end{table}

\if false
\begin{table}
    \begin{center}
    \setlength{\tabcolsep}{2.5pt}
    \begin{tabular}{ccccc}
    \toprule[1pt]
    $l_b$ & Acc ($\%$) $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    \hline
   4 & 96.48 & 39.88 & 0.9938 & 0.0103 \\
   8 & 97.28 & 40.70 & 0.9940 & 0.0087 \\
   16 & 96.07 & 38.36 & 0.9898 & 0.0149 \\
   32 & 83.71 & 35.59 & 0.9767 & 0.0402 \\
    \hline
    % $\checkmark$ & $\checkmark$ & 16 & 96.07 & 38.36 & 0.9898 & 0.0149 \\
    % \hline
    \toprule[1pt]
    \end{tabular}
    \end{center}
    \vspace{-10pt}
    \caption{The model performance under various message length $l_b$
    \ca{separate, only length}
    }
\label{tab.ablation_studies}
\vspace{-6pt}
\end{table}
\fi

\if false
\begin{table}
    \centering
    \setlength{\tabcolsep}{4pt} % Adjust column spacing
    \renewcommand{\arraystretch}{1.2} % Keep row height fixed
    \newcolumntype{Y}{>{\centering\arraybackslash}X} % Centered columns in tabularx
    \newcolumntype{Z}{>{\centering\arraybackslash}p{2.2cm}} % Wider column for Acc (%)
    \begin{tabularx}{\columnwidth}{Y Z Y Y Y}  % Allocate more width to Acc (%)
    \toprule[1pt]
    $l_b$ & Acc ($\%$) $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    \midrule
    4  & 96.48  & 39.88  & 0.9938  & 0.0103 \\
    8  & \textbf{97.28}  & \textbf{40.70}  & \textbf{0.9940}  & \textbf{0.0087} \\
    16 & 96.07  & 38.36  & 0.9898  & 0.0149 \\
    32 & 83.71  & 35.59  & 0.9767  & 0.0402 \\
    64 & 62.50 & 22.65 & 0.8658 & 0.1662 \\
    128 & 53.90 & 30.29 & 0.9652 & 0.0668 \\
    \bottomrule[1pt]
    \end{tabularx}
    \vspace{-6pt}
    \caption{The model performance under various message lengths $l_b$ \textit{(separate, only length)}.}
    \label{tab.ablation_studies}
\end{table}
\fi

% \begin{figure}
%   \centering
%    \includegraphics[width=0.8\linewidth]{Figs/lb_vs_acc_psnr.pdf}
%    \caption{The model performance under various message lengths $l_b$ \textit{(separate, only length)}.}
%    % \ca{1) more views, 2) render only markers}
%   \label{fig:ablation_studies}
%   %\vspace{-10pt}
% \end{figure}


\if false
\begin{figure*}[ht]
  \centering
  \begin{subfigure}[t]{0.24\textwidth}  % Force alignment to the top
    \centering
    \includegraphics[width=\linewidth]{Figs/Training_Loss.pdf}
    \caption{Training loss of the models under various settings. ``Fix'', ``PLA'', and ``LA'' denote three types of learnable perturbation amplitude settings: fix amplitude, partial learnable amplitude, learnable amplitude.}
    \label{fig:training_loss}
  \end{subfigure}%
  \hfill
  \begin{subfigure}[t]{0.335\textwidth}  % Force alignment to the top
    \centering
    \includegraphics[width=\linewidth]{Figs/lb_vs_acc_psnr.pdf}
    \caption{The model performance under various message lengths $l_b$ \textit{(separate, only length)}.}
    \label{fig:bit_length}
  \end{subfigure}
  \vspace{-8pt}
\end{figure*}
\fi




\paragraph{Message length.}
% We conduct a series of experiments on message length $l_b \in \{4, 8, 16, 32\}$ to investigate the relationship between model performance and message length. As illustrated in \cref{tab.ablation_studies}, the bit accuracy decreases when the message length increases to $32$. Nevertheless, the bit accuracy remains above $90\%$ for all message lengths below $32$, suggesting that the model maintains a high level of accuracy when encoding shorter messages. Furthermore, it is important to note that the visual quality of the rendered outputs does not degrade as the message length increases. This observation underscores the effectiveness of our encoder in preserving visual fidelity. 
% We conduct a series of experiments on various message lengths $l_b$ to investigate the relationship between model performance and message length. As illustrated in \cref{fig:ablation_studies}, the performance of our model decreases when the message length increases to $32$. However, when the message length is lower than $32$, our model can achieve admirable bit accuracy and visual quality. 

We conduct a series of experiments to analyze the impact of message length $l_b$ to explore the embedding capacity of our model.
As shown in \cref{fig:ablation_studies}, both bit accuracy and visual quality decline as $l_b$ increases beyond 32. 
For shorter message ($l_b < 32$), our model maintains high accuracy and good visual quality. This indicates that while longer messages introduce more embedding complexity, moderate message lengths strike a balance between watermark robustness and rendering fidelity.



% the bit accuracy decreases when the message length increases to $32$. However, 
% the bit accuracy remains above $90\%$ for all message lengths below $32$, indicating that the model maintains a high level of accuracy when encoding shorter messages. Furthermore, the visual quality of the rendered images does not degrade significantly as the message length increases, demonstrating the effectiveness of our encoder in preserving visual fidelity. 
% \begin{table}
%     \begin{center}
%     \begin{tabular}{ccccc}
%     % \begin{tabularx}{\textwidth}{XXXXX}
%     % \begin{tabular}{p{2.2cm}p{1.3cm}p{1.1cm}p{1.1cm}p{1.1cm}}
%     \toprule[1pt]
%      $l_b$ & Acc ($\%$) $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
%     \hline
%     4 & 96.48 & 39.88 & 0.9938 & 0.0103 \\
%     \hline
%     8 & 97.28 & 40.70 & 0.9940 & 0.0087 \\
%     \hline
%     16 & 96.07 & 38.36 & 0.9898 & 0.0149 \\
%     \hline
%     32 & 75.29 & 42.78 & 0.9944 & 0.0076 \\
%     \toprule[1pt]
%     \end{tabular}
%     \end{center}
%     \caption{Bit accuracies and visual qualities of our methods on various message length.}
%     % \ca{acc is too low for 32bits}}
% \label{tab.performance_vs_message_len}
% \end{table}
% \subsection{Ablation Study}

% \paragraph{Ablation on decoder.}
% We pretrain the decoder on the render images of 3D object as mention in \cref{sec.method_2D_decoder}. 
% % To analyze the role of pretraining decoder, we compare the performance of our method with and without pretraining the decoder. 
% \cref{tab.ablation_studies} demonstrates that the bit accuracy of the framework with random initialized decoder is much lower than that with pretraining decoder. This results illustrate that the pretraining process of decoder can improve the performance of the 3D watermarking framework.

% \begin{table}
%     \begin{center}
%     \setlength{\tabcolsep}{2.5pt}
%     \begin{tabular}{ccccc}
%     \toprule[1pt]
%      & Bit Acc ($\%$) $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
%     \hline
%     w/ Pretraining & 96.07 & 38.36 & 0.9898 & 0.0149 \\
%     \hline
%     w/o Pretraining & 83.84 & 37.57 & 0.9893 & 0.0185 \\
%     \toprule[1pt]
%     \end{tabular}
%     \end{center}
%     \caption{Bit accuracies and visual qualities of our methods with and without pretraining the 2D decoder on Gobjaverse dataset. The experiments are conducted on message length $l_b=16$.}
% \label{tab.ablation_decoder}
% \end{table}

% \paragraph{Ablation on input normalization strategy.} 
% We conduct comparative experiments on our framework with and without application of the input normalization strategy discussed in \cref{sec.method_3D_encoder}. 
% % This normalization process involves normalizing the coordinates, scaling, rotation, opacity, and color of the Gaussian primitives to the interval $[-1, 1]$. 
% As ilustrated in \cref{tab.ablation_studies}, our method with input normalization demonstrates better performance compared to the framework that without normalization. 
% % A possible explanation for this improvement is that the normalized input facilitate more efficient and stable model training, making the model more effective and easier to train.

% \begin{table}
%     \begin{center}
%     % \setlength{\tabcolsep}{2.5pt}
%     \begin{tabular}{ccccc}
%     \toprule[1pt]
%      & Bit Acc ($\%$) $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
%     \hline
%     w/ IN & 96.07 & 38.36 & 0.9898 & 0.0149 \\
%     \hline
%     w/o IN & 95.88 & 37.89 & 0.9899 & 0.0169 \\
%     \toprule[1pt]
%     \end{tabular}
%     \end{center}
%     \caption{Bit accuracies and visual qualities of our methods with and without input normalization (IN). The experiments are conducted on message length $l_b=16$.}
% \label{tab.ablation_norm_input}
% \end{table}

% \subsection{Distortion}
% We conduct a comprehensive evaluation of the robustness of the proposed WaterGS algorithm against various distortions, as described in Section~\ref{sec.method_distortion_layer}. The experimental results are summarized in Table~\ref{tab.distortion}. As illustrated in the table, our method demonstrates a high degree of resilience across a diverse range of distortion types, which underscore the effectiveness of our approach in handling real-world scenarios where such distortions are prevalent.
% \begin{table}
%     \begin{center}
%     \setlength{\tabcolsep}{2.5pt}
%     \begin{tabular}{c|c}
%     % \begin{tabularx}{\textwidth}{XXXXX}
%     % \begin{tabular}{p{2.2cm}p{1.3cm}p{1.1cm}p{1.1cm}p{1.1cm}}
%     \toprule[1pt]
%      Distortion Type & Bit Acc $(\%)$ $\uparrow$ \\
%     \hline
%     No Distortion & 97.72 \\
%     Crop & 82.71  \\
%     Dropout & 96.03  \\
%     JPEG Compression & 94.60  \\
%     \toprule[1pt]
%     \end{tabular}
%     \end{center}
%     \caption{Bit accuracy under various distortions.}
% \label{tab.distortion}
% \end{table}

% \subsection{Discussion}
% \paragraph{View variance.}
% To analyze the robustness of our method and other baseline methods against camera pose variations, we assess the standard deviation of bit accuracy across multiple views of the same object. For each object in our test dataset, we randomly sample 40 camera poses and calculate the bit accuracy for each pose. Subsequently, we compute the standard deviation of these bit accuracy for each object and averaged these values across the dataset. The experimental results indicate that the standard deviation of bit accuracy for our method and WateRF are $4.00\%$ and $7.17\%$, respectively. While the average bit accuracy of our method and WateRF are $96.07\%$ and $85.27\%$. This experimental results underscores the enhanced robustness of our method to variations in camera poses.

% is demonstrated in \cref{tab.bit_std}.We observe that our method achieves a lower standard deviation, which underscores the enhanced robustness of our method to variations in camera poses.
% \begin{table}
%     \begin{center}
%     \setlength{\tabcolsep}{2.5pt}
%     \begin{tabular}{ccc}
%     \toprule[1pt]
%      & Bit Acc mean ($\%$)  & Bit Acc std ($\%$)  \\
%     \hline
%     Ours & 96.07 & 4.00 \\
%     \hline
%     WateRF & 80.38 & 7.17 \\
%     \toprule[1pt]
%     \end{tabular}
%     \end{center}
%     \caption{The mean value and standard deviation of bit accuracy. The experiments are conducted on message length $l_b=16$}
% \label{tab.bit_std}
% \end{table}

\subsection{Distortion impact.}
% We conduct a comprehensive evaluation of the robustness of the proposed WaterGS algorithm against various distortions.
% The results in \cref{tab.distortion} illustrate that our method is robust against a diverse range of distortion types.


We evaluate the robustness of the proposed \ours~method against various distortions, as presented in \cref{tab.distortion}. 
The results demonstrate that our method maintains high bit accuracy across a wide range of both 2D and 3D distortions. While minor variations exist among different distortion types, the overall performance remains stable, indicating strong resilience. Notably, the model achieves 96.03\% accuracy under dropout distortion (2D) and 96.31\% under crop distortion (3D), further confirming its robustness in challenging conditions.



% which underscore the effectiveness of our approach in handling real-world scenarios where such distortions are prevalent.
% \begin{table}
%     \begin{center}
%     \setlength{\tabcolsep}{2.5pt}
%     \begin{tabular}{c|c}
%     % \begin{tabularx}{\textwidth}{XXXXX}
%     % \begin{tabular}{p{2.2cm}p{1.3cm}p{1.1cm}p{1.1cm}p{1.1cm}}
%     \toprule[1pt]
%      Distortion Type & Bit Acc $(\%)$ $\uparrow$ \\
%     \hline
%     No Distortion & 97.72 \\
%     % Crop & 82.71  \\
%     Crop & 94.77  \\
%     Dropout & 96.03  \\
%     JPEG Compression & 94.60  \\
%     \toprule[1pt]
%     \end{tabular}
%     \end{center}
%     \caption{Bit accuracy under various distortions.}
% \label{tab.distortion}
% \end{table}

% \begin{table}
%     \begin{center}
%     % \setlength{\tabcolsep}{2.5pt}
%     \begin{tabular}{cccc}
%     % \begin{tabularx}{\textwidth}{XXXXX}
%     % \begin{tabular}{p{2.2cm}p{1.3cm}p{1.1cm}p{1.1cm}p{1.1cm}}
%     \toprule[1pt]
%      No Distortion & Crop & Dropout & JPEG \\
%     \hline
%     97.72 & 94.77 & 96.03 & 94.60 \\
%     \toprule[1pt]
%     \end{tabular}
%     \end{center}
%     \vspace{-10pt}
%     \caption{Bit accuracy under various distortions.}
% \label{tab.distortion}
% \vspace{-12pt}
% \end{table}

\begin{table}[htbp]
    \begin{center}
    \setlength{\tabcolsep}{1.5pt}
    % \renewcommand{\arraystretch}{0.9}
    \small
    \resizebox{0.99\linewidth}{!}{

    \begin{tabular}{c|ccccc|cc}
    % \begin{tabularx}{\textwidth}{XXXXX}
    % \begin{tabular}{p{2.2cm}p{1.3cm}p{1.1cm}p{1.1cm}p{1.1cm}}
    \toprule[1pt]
       \multirow{2}{*}{None}  & \multicolumn{5}{|c|}{\textbf{2D Distortion}} & \multicolumn{2}{c}{\textbf{3D Distortion}} \\
      & \makecell{Crop \\[-3pt] \scriptsize $cr=0.4$} & \makecell{Dropout \\[-3pt] \scriptsize $p=0.1$} & \makecell{JPEG \\[-3pt] \scriptsize $Q=50$}  & \makecell{Rotation \\[-3pt] \scriptsize $r=\pm30^{\circ}$} & \makecell{Noise \\[-3pt] \footnotesize $\sigma=0.06$}  & \makecell{Dropout \\[-3pt] \scriptsize $p=0.2$} & \makecell{Cropout \\[-3pt] \scriptsize $cr=0.4$} \\
    \hline
    97.67 & 95.02 & 96.03 & 94.60 & 96.77 & 96.54 & 95.91 & 96.31 \\
    \textit{Delta} & \textit{-2.65} & \textit{-1.64} & \textit{-3.07} & \textit{-0.90} & \textit{-1.13} & \textit{-1.76} & \textit{-1.36} \\
    
    \toprule[1pt]
    \end{tabular}         
    }
    \end{center}
    \vspace{-20pt}
    \caption{Bit accuracy under various distortions.}
\label{tab.distortion}
\vspace{-15pt}
\end{table}




==> sec/cvpr_rules.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/draft.tex <==

\cb{

\section{Experiment}
\subsection{Analysis of learnable amplitude}

% The exponential term $E$ governs the spatial falloff; if the pixel is far from the Gaussian center, the contribution (and hence the gradient) decays exponentially.
Opacity and color influence the gradient linearly.
Position gradients scale with the distance from the center, normalized by the spread of the Gaussian.
Scale and orientation gradients are more sensitive, as they depend on the squared distance and are scaled by $\sigma^{-4}$, meaning that changes in these parameters can have a dramatic effect, especially for Gaussians with a small spread.
This analysis provides insight into how each property contributes to the gradient during differentiable rendering in a 3DGS framework.

}

==> sec/w_marker.tex <==

% \noindent \textbf{W-Markers initialization.} 
% \paragraph{W-Markers Proposal.}
\subsection{Adaptive Marker Control}
\label{sec.W-Marker}
% pre-process the input Gaussian splatting. The W-Maker initialization process adds a batch of random Gaussian primitives into the input Gaussian splatting, which we name as W-Marker. 
% propose to add W-Markers that consisted of a batch of random Gaussian primitives into the input Gaussian splatting to enhance message embedding.
% We introduce $N_r$ random Gaussian primitives, named as W-Marker, into the input Gaussian splatting in order to emhance message embedding. 
% We propose a W-Markers initialization process to incorporate random texture into the input Gaussian splatting. This design is motivated by findings from several studies indicating that encoder-decoder based watermarking frameworks for 2D images typically embed watermark messages into high-level features of the input, such as the texture or edge \cite{}. We hypothesize that this observation is equally applicable to 3D watermarking. However, when the surface of the input Gaussian splatting is smooth or lacks sufficient texture, the encoder may struggle to embed the watermark message into the 3DGS, resulting in the failure of the decoder to extract the message from rendered image. Therefore, we propose W-Markers initialization process to address this problem. This process introduce the proposed W-Maker that consisted of random Gaussian primititivs into the input Gaussian splatting, thereby enriching the surface texture and enhancing the encoder's embedding capabilities.

In the embedding process, we introduce a specially designed random Gaussian splatting, named W-Markers, into the input Gaussian splatting to facilitate the watermark embedding. This design is motivated by the insight from existing studies on digital watermarking, which points out that the watermarking frameworks for 2D images typically embed watermark into high-level features of the input, such as the texture or edge \cite{high_freq}.
% findings from several studies indicating that encoder-decoder based watermarking frameworks for 2D images typically embed watermark messages into high-level features of the input, such as the texture or edge \cite{high_freq}. 
We hypothesize that this observation is equally applicable to 3D watermarking. 
% and propose the W-Markers to take advantage of this finding.
% However, when the surface of the input Gaussian splatting is smooth or lacks sufficient texture, the encoder may struggle to embed the watermark message into the 3DGS, resulting in the failure of the decoder to extract the message from rendered image. 
% Therefore, we propose W-Markers to introduce more texture into the input 3DGS for facilitating the message embedding. 
In the embedding process, we integrate the W-Markers into the input 3DGS. This addition enriches the surface texture, thereby facilitating the watermark embedding.
 
For generating W-Markers, we begin by randomly sampling a minimal batch of Gaussian primitives from the input 3DGS, with the number of sampled primitives being $p_s \ (p_s < 1)$ times the total number of primitives in the input 3DGS. Each selected primitive is then subdivided into $N_{split}$ smaller Gaussian primitives. The center positions of the new primitives are set near the original primitive, while the scaling factors are reduced. Additionally, the opacity, rotation, and color of the new primitives are randomly assigned. This procedure generates a new Gaussian splatting with $N_r=p_s \cdot N \cdot N_{split}$ primitives, which serve as the W-Markers in our embedding pipeline. 


To further enhance the encoder's adaptability to the W-Markers, we introduce learnable weights $w_s$ and $w_\alpha$ for the scaling factor and opacity respectively of the Gaussian primitives within the W-Markers. Therefore, the scaling factor $s'$ and opacity $o'$ of a new Gaussian primitive in the W-Markers are calculated as follows:
\begin{equation}
\begin{split}
    s' &= \frac{s}{1.6} \times w_s \\
    o' &= \text{rand}(0,1) \times w_\alpha
\end{split}
\label{split_GS}
\end{equation}
where $s$ denotes the scaling factor of the original primitive from which the new primitive is derived, and $\text{rand}(0,1)$ represents a random value uniformly sampled from the interval $[0, 1]$. The learnable weights $w_s$ and $w_\alpha$ are shared across all primitives in the W-Markers. The resulting W-Markers is then integrated with the input 3DGS, culminating in a merged textured 3DGS $G_{tex}(M_{tex}, S_{tex}, R_{tex}, C_{tex}, A_{tex})$ with a total of $N+N_r$ primitives. 

\todolj{
+ an illustration figure
1. select, 
2. perturbation range, learnable weighting.

}

\paragraph{Adaptive weighting.}
% \ca{add weighting stretagy}
To ensure optimal training coverage, we design an adaptive weighting strategy that dynamically adjusts the weights of message loss ($W_{msg}$) and image loss ($W_{img}$) in the training process. Our model is designed to initially focus on embedding the watermark message and subsequently enhance the visual quality of the watermarked 3DGS. Consequently, the adaptive strategy is structured into three stages. In the first stage, we initialize $W_{msg}$ at a relatively high value of $80$, while $W_{img}$ is set to a minimal value of $0$. During this stage, $W_{msg}$ is linearly reduced to $1$, while $W_{img}$ is linearly increased to $1$. 
% This approach prioritizes learning the watermark embedding initially, shifting focus gradually towards maintaining image quality. 
In the second stage, both $W_{msg}$ and $W_{img}$ are fixed at 1. This setting is maintained to simultaneously optimize both the bit accuracy and the visual quality of the images. In the final stage, $W_{img}$ is linearly increased from $1$ to $2$ for improving the visual quality further.
% in this stage. This adjustment allows for finer improvements in the rendered images aesthetics without compromising the embedded watermark.

Additionally, the learnable weights $w_s$ and $w_\alpha$ of the W-Markers introduced in \cref{sec.W-Marker} follow an update pattern aligned with these stages. Specifically, $w_s$ and $w_\alpha$ are maintained at their initial values in the first two stages and are updated in the final stage. We experimentally find this strategy helps improve the visual quality of our model.
% Additionally, we adopt the update strategy for the learnable weights $w_s$ and $w_\alpha$ of the W-Markers introduced in \cref{sec.W-Marker} during the three stages of the adaptive weighting strategy. Specifically, $w_s$ and $w_\alpha$ are maintained at their initial values without updates in the first two stages, and are updated in the final stage. We experimentally find this update strategy is beneficial for improving the visual quality of our model.

